A Parallel Approximation Algorithm for Maximizing Submodular $b$-Matching

We design new serial and parallel approximation algorithms for computing a maximum weight $b$-matching in an edge-weighted graph with a submodular objective function. This problem is NP-hard; the new algorithms have approximation ratio $1/3$, and are relaxations of the Greedy algorithm that rely only on local information in the graph, making them parallelizable. We have designed and implemented Local Lazy Greedy algorithms for both serial and parallel computers. We have applied the approximate submodular $b$-matching algorithm to assign tasks to processors in the computation of Fock matrices in quantum chemistry on parallel computers. The assignment seeks to reduce the run time by balancing the computational load on the processors and bounding the number of messages that each processor sends. We show that the new assignment of tasks to processors provides a four fold speedup over the currently used assignment in the NWChemEx software on $8000$ processors on the Summit supercomputer at Oak Ridge National Lab.

==> acda-review.tex <==
SUBMISSION: 57
TITLE: A Parallel Approximation  Algorithm for Maximizing Submodular b-matching


----------------------- REVIEW 1 ---------------------
SUBMISSION: 57
TITLE: A Parallel Approximation  Algorithm for Maximizing Submodular b-matching
AUTHORS: S M Ferdous, Arif Khan, Alex Pothen, Ajay Panyala and Mahantesh Halappanavar

----------- Overall evaluation -----------
This paper proposes a parallel algorithm for maximizing a monotone submodular function under a b-matching constraint. The authors make an assumption that the marginal gain of the objective function relies only on the adjacent edges (Assumption 4.1). Under this assumption, they propose a non-parallel algorithm called the Local Lazy Greedy algorithm, which runs in O(\beta m \log \Delta) time, where \beta is the largest degree of the feasible b-matching and \Delta is the largest degree of the underlying graph. They also show that the Local Lazy Greedy algorithm can be parallelizable and empirically validate its efficiency with a load balancing problem.

Overall, this paper is clearly written. The problem of maximizing a monotone submodular function under a b-matching constraint is an important problem since it has many applications in social networks, bioinformatics, and natural language processing. Also, this paper adds a new application to load balancing for Fock matrix computation. This paper proposes the first parallel algorithm for this problem, which is a nice contribution and has many potential applications.

In my opinion, it would be better to add more explanations of Assumption 4.1 in the abstract and introduction section. The current version of the manuscript seems to mention this assumption only on page 2 ("Under suitable assumptions"). Since this is a natural but significant assumption, the authors should mention what is this assumption and explain that natural objective functions such as (2.2) satisfy this assumption in the abstract and introduction section. 
%%% smf: edited to reflect the comment.

Also, it would be helpful if this assumption is mentioned in Table 1.
%%%smf: Mentioned in the table.

%%%%% References%%%%%
My other concern is about the references. This paper mentions the most important existing results but sometimes seems to cite an incorrect paper. For example,
- In the related work section, this paper cites [9] as a reference for the term "k-independence systems". However, this word was not used in [9]. [9] calls this notion "k-systems". I think most existing papers call it "k-systems", so it would be better to use the term "k-systems".
- (1-1/e)-approximation of the greedy algorithm was proved by [31], not [17].
- The tightness of the (1-1/e)-approximation was proved by the following paper in my understanding, not [8].
        GL Nemhauser, LA Wolsey. Best algorithms for approximating the maximum of a submodular set function. Math of OR, 1978.
- The 1/2-approximation greedy algorithm for SWM was proved by [23], not by [37].
- The fact that the running time of the Lazy Greedy is no better than the Greedy was first mentioned by [28], not by [29].
If the authors address these points, I would like to weakly recommend the acceptance of this paper.
%%%smf: corrected the references.
Minor comments:
- page 1: "b-matching may be viewed as the relaxation of a matroid, called a 2-extendible system" might not be precise. It might be replaced with "b-matching may be viewed as a special case of a 2-extendible system, which is a generalization of a matroid".
%%% smf: replaced.
- In the last part of page 2, what is W in the definition of b-matching constraints? Here the objective function is a set function, and not related to the weights of edges.
%%%-smf: W is the weights on the edges. Submdoular function is defined on the set of edges , and weight function is one to one function on the edges. 
- To make the objective function of (2.2) submodular, \alpha should be assumed to be in [0, 1].
%%%smf: added
- page 3: A greedy algorithm that repeatedly chooses a set -> A greedy algorithm that repeatedly chooses an element
%%%smf: replaced
- page 3: The running time of the randomized local search is O(\beta^{p+1} (\Delta - 1)^p m \log(1/\epsilon)), not O(\beta^{p+1} (\Delta - 1)^p m \log(1/\epsilon)). Also, it would be better to mention its approximation ratio 1/(2+1/p+\epsilon).
%%%smf: the comment has a flaw. I have updated the correct one in the paper. 
- page 4: b-constraints -> b-matching constraints
%%% smf: replaced
- page 7: The paragraph starting with "In line 2" explain inequalities and equalities, but the authors count all of them as inequalities.
%%% smf: this comes directly from proposition 2.2. I have referred proposition \ref{prop:monotone}. 



----------------------- REVIEW 2 ---------------------
SUBMISSION: 57
TITLE: A Parallel Approximation  Algorithm for Maximizing Submodular b-matching
AUTHORS: S M Ferdous, Arif Khan, Alex Pothen, Ajay Panyala and Mahantesh Halappanavar

----------- Overall evaluation -----------
This paper considers the submodular b-matching problem.  In the problem, one is to construct a b matching. Then each element of the matching is fed into a submodular function.  The goal is to choose the matching to optimize the submodular function.

This is a natural and interesting problem. 

There has been a lot of interest in problems like this. For this problem, approximation algorithms are known.  Further, the lazy greedy algorithm is known to create a good approximate solution efficiently.

This paper considers the problem in the parallel setting for, what I think, is the first time.  They show how to make the lazy greedy algorithm concurrent so that it is highly parallelizable.  This is a nice contribution.  They are able to do this without losing the in approximation guarantee.

They give experiments demonstrating the scalability of the algorithm. These experiments back up the theoretical results and show that they can be used in practice.

Overall, this seems like a good paper for ACDA.  Solid theory on an important problem.  The theory is non-trivial but close to prior work.  The experiments are promising and validate the theoretical results.



----------------------- REVIEW 3 ---------------------
SUBMISSION: 57
TITLE: A Parallel Approximation  Algorithm for Maximizing Submodular b-matching
AUTHORS: S M Ferdous, Arif Khan, Alex Pothen, Ajay Panyala and Mahantesh Halappanavar

----------- Overall evaluation -----------
This paper presents an approximation algorithm for submodular b-matching based on a (locally) greedy strategy. The algorithm is shown to be correct and experiments verify that it is more efficient than a local greedy variant both when run sequentially and in parallel. Finally, the algorithm is used to load balance a parallel application involving quantum chemistry computations.

The paper is well written and fairly easy to follow, although one could wish that the experimental section contained more detail. This might be due to the page limit. It should be interesting for the ACDA community in that it develops a non-trivial efficient (parallel) combinatorial algorithm
and shows how it can be used to speed up a scientific application.

However, there exists (at least) one previous study of parallel b-matching algorithms, "Efficient Approximation Algorithms for Weighted $b$-Matching" in SIAM J. Sci. Comput., 38(5), S593–S619 by Khan et al. Although different, this algorithm has resemblances to the presented algorithm
in that it also computes dominant edges. This paper is neither referenced nor is the presented algorithm compared against this. This is somewhat odd.

Some questions:

Setting b(v) = |U|/|V| seems to limit the possibility for load balancing. Point in case, if the cost of the first job in Figure 1 is increased to 400, then this would force a partitioning as (400,50) and (200,100) as opposed to (400) and (200,100,50). It is later stated, at the end of Section 3, "in our problem we are required to set an upper bound on the individual partition sizes." but this is never justified.
%%%smf: need to address this. 

On page 5 just below Algorithm 1, should "\beta n" not be "\beta n/2" since each selected edge joins two vertices?
%%%smf: Yes. We wrote bounded by and it does not change the complexity anywhere. 

Minor comments:

2.1 The term V is used both for defining a submodular function and later for the vertices of the graph.
%%%smf: replaced V and U with X as ground set. U and V are kept only for vertex set.
Top of page 3. Note that f was not used in the preceeding definition and not in the following either (2.2).
%%%smf: f is used as a submodular function throughout the background section. Changed from Z to f of equation 2.2.

Page 3, (2.2) alpha is not defined.
%%%smf: corrected 


----------------------- REVIEW 4 ---------------------
SUBMISSION: 57
TITLE: A Parallel Approximation  Algorithm for Maximizing Submodular b-matching
AUTHORS: S M Ferdous, Arif Khan, Alex Pothen, Ajay Panyala and Mahantesh Halappanavar

----------- Overall evaluation -----------
The authors propose approximation algorithms to compute a maximum weight b-matching in an edge-weighted graph with a submodular objective function.

+ While not well-organized, the paper does provide a good explanation of the proposed algorithms and the results are demonstrated on a large number of datasets.

- The paper is hard to follow and needs to be restructured. I recommend putting all the contributions in one section with subsections and moving the related works to the end of the paper. The motivation and background section can discuss the main related work that helps understand the contributions of the work.  Section 2 needs a topic paragraph and section 2.1 should not start with a definition.


-The results are not compared to prior work.

==> extra.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=\columnwidth]{fig/uracil_1222_240_0.5_1_weight.pdf}
    \caption{total weight of the loads per machine for $\alpha=1$ (up) and $\alpha = 0.5$ (down)}
    \label{fig:load_balance}
\end{figure}


\begin{table}[H]
\centering
\begin{tabular}{l|ll}
\hline
           & $\alpha = 1$                 & $\alpha = 0.5$               \\
           \hline
avg weight & 2667.29 & 2666.87 \\
std weight & 1071.45 & 46.63   \\
max weight & 5191.98 & 2757.63 \\
min weight & 3.49    & 2590.55\\
Coeff. Var. & 0.4017 &	0.0175 \\
\hline
\end{tabular}
\caption{Statistics for the load balance dataset}
\end{table}

\begin{figure}[H]
    \centering
    \includegraphics[width=\columnwidth]{fig/c60_139650_240_0.5_1_weight.pdf}
    \caption{total weight of the loads per machine for $\alpha=1$ (up) and $\alpha = 0.5$ (down)}
    \label{fig:load_balance}
\end{figure}


\begin{table}[H]
\centering
\begin{tabular}{lrr}
\hline
            & $\alpha = 1$ & {$\alpha = 0.5$} \\
            \hline
avg weight  & 33504032.50                      & 33503871.25                        \\
std weight  & 6868411.64                       & 29865.28                           \\
max weight  & 49975900.00                      & 33582100.00                        \\
min weight  & 25019500.00                      & 33450700.00                        \\
Coeff. Var. & 0.2050                           & 0.0009                             \\
time (sec.) & 19.37                            & 232.80       \\
\hline

\end{tabular}
\end{table}

\begin{figure}[H]
    \centering
    \includegraphics[width=\columnwidth]{fig/c60_139650_1200_0.5_1_weight.pdf}
    \caption{total weight of the loads per machine for $\alpha=1$ (up) and $\alpha = 0.5$ (down)}
    \label{fig:load_balance}
\end{figure}

\begin{table}[H]
\centering
\begin{tabular}{lrr}
\hline
            & $\alpha = 1$ & {$\alpha = 0.5$} \\
            \hline
avg weight  & 6700815.24                       & 6700813.51                         \\
std weight  & 3580473.87                       & 2785.12                            \\
max weight  & 13413600.00                      & 6709760.00                         \\
min weight  & 1074340.00                       & 6693690.00                         \\
Coeff. Var. & 0.5343                           & 0.0004                             \\
time (sec.) & 90.07                            & 929.70           \\
\hline

\end{tabular}
\end{table}

==> nsf-propsal.tex <==
\section{Introduction}
Let $f$ be a set function defined on the powerset of a set $V$, $f:2^V\xrightarrow{}R $. 
Then $f$ is submodular if for every $A \subseteq B \subseteq V$ and $e \in V\setminus B$, we have  $f(A \cup e)-f(A) \geq f(B \cup e) - f(B)$.
Informally submodularity ensures diminishing marginal gain. 
Moreover, $f$  is monotone if for every $A \subseteq B \subseteq V$, $f(A) \leq f(B)$. Submodular functions naturally arise in several applications such as coverage and weighed coverage functions, facility location, entropy and mutual information \cite{Krause14}.

Maximizing a monotone submodular function with constraints is NP-hard in general. In fact it is NP-hard even for the simplest constraint, i.e., cardinality,  for many classes of submodular functions \cite{Feige98,Krause05}. A greedy algorithm that chooses repeatedly a set with maximum marginal gain is known to achieve $(1-1/e)$ approximation ratio \cite{Fisher1978}. This approximation ratio is known to be tight \cite{Buchbinder14}. A survey on submodular function maximization under different constraints can be found in \cite{Krause14}.

We are interested in optimizing submodular functions on a graph. A number of natural class of constraints arise in that case.  We  focus in particular on \bmatching \  and \bedgecover \  constraints. Recall that $G(V,E)$ denotes an undirected graph where $V$ and $E$ are the set of vertices and edges, respectively, and let  $b \in Z^{|V|}$ denote positive integer capacities for the degree of each vertex. 
%A \bmatching \  is a subset of edges $M$ such that at most $b(v)$ edges in M are incident on each vertex v. Note that \bmatching \  generalizes the matching problem, where $b(v)$ is identically equal to one for each $v\in V$. 
In the following we will denote  $\beta = \text{max}_{v \in V}b(v)$.

\subsection{Recent Progress}
A subset system is a pair $(U,I)$, where $U$ is a finite set of elements and $I$ is a collection of subsets (commonly called independent sets) of $U$ with the property that if $A \in I$ and $A' \subseteq A$ then $A' \in I$. A matroid is a subset system $(U,I)$ which satisfies the  property that 
$\forall A,B \in I$ and $|A|<|B|$,  $\exists e \in B \setminus A$ such that $A+e \in I$. A subset system $(U,I)$ is  a $k$-independence system \cite{Calinescu11} for an integer $k\geq 1$ if for every $A \in I$ and $e \in U$, there exists a set $B \subseteq A$ such that $|B| \leq k$ and $A\setminus B + e \in I$. It is also known as a $k$-system~\cite{Feldman11}. The Greedy algorithm for maximizing a monotone submodular function with matroid constraints achieves  1/2-approximation ratio. More generally with k-matroid intersection and $k-$independence system constraints,  the approximation ratio is $1/(k+1)$ \cite{Calinescu11}. 
%This ratio also remains the same for $k-$independence system constraints. \cite{Calinescu11,jenkyns}.
%define k-exchange system.
Max $k$-cover can be reduced to submodular \bmatching\  \cite{Fuji16}.  \cite{Feige98} showed that there is no polynomial time algorithm for approximating the max $k$-cover within a factor of $(1-1/e+\epsilon)$ for any $\epsilon > 0$. Thus we obtain an  immediate bound on the approximation ratio of submodular \bmatching. % , i.e., $(1-1/e)$. 
%(I did not figure out the reduction but have some idea how it may work)

Several approximation algorithms have been proposed for maximizing monotone submodular functions with \bmatching\  constraints. If the graph is bipartite, then the \bmatching \  constraint can be represented as the intersection of two partition matroids, and  the Greedy algorithm  provides $1/3$-approximation ratio. \bmatchings \  in non-bipartite graphs are not thus representable as the intersection of partition matroids \cite{Fekete2003}. Nevertheless as  \bmatching \  forms a $k-$system, the Greedy algorithm  yields a $1/3$-approximation ratio  for non-bipartite graphs.  \cite{Feldman11} showed that \bmatching \  is also a $k$-exchange system, and  they provide a $1/(2+\frac{1}{p}+\epsilon)$-approximation algorithm based on local search, with  runtime $O(\beta^{p+1} (\Delta-1)^p nm\epsilon^{-1})$. 
(Here $p$ is a parameter to be chosen.) 
Recently \cite{Fuji16} developed two algorithms for the problem. One of them has the approximation ratio of  $1/4$,  but it is  faster than the classical Greedy algorithm. The other algorithm is a faster variant of the local search algorithm from \cite{Feldman11}.

%\chg{

Minimizing a submodular function is solvable in strongly polynomial time \cite{Iwata01}, but the addition of constraints make the problem harder \cite{Svitkina11}. A particular type of constraint that has  attracted interest is the covering constraint \cite{Wolsey82,Koufogiannakis13,Iwata09}. Let $U$ be a finite set of $n$ elements and $ S= \{S_1,\dots ,S_n\}$ be a collection of subsets of $U$. Let $\eta$ be the maximum frequency of an element in the subsets of $S$. A set cover is the problem of selecting as few subsets as possible from $S$ such that their union covers  $U$. If there are non-negative costs associated with the elements of $S$, the problem is to find a cover with minimum total cost. The set cover problem with linear cost function is NP-hard, and in fact set cover can not be approximated efficiently beyond $o(\log n)$ \cite{Feige98}. 
%A set cover generalizes several important combinatorial problems such as vertex cover and edge cover in graphs.
%For vertex cover the covering elements are the edges and the collection of subsets are the incident edges for each vertex. Conversely for edge cover, the covering elements are the vertices and collection of subsets are simply the edges. 
In the classic covering problems, each element needs to be covered by at least one of the subsets. We can generalize the covering requirement to a positive integer value to obtain the  set multicover problem. 
%The edge cover with the covering requirement of $b(v)$  for each vertex $v$  is the \bedgecover \  problem. 

We are interested in covering problems where the cost function is submodular. For the general set cover problem, there is an $\eta$-approximation algorithm\cite{Iwata09}. This amounts to  $2$-approximation algorithm for vertex cover and $\Delta$-approximation algorithm for edge cover. 
%($\Delta$ is the maximum degree of a vertex.)  
There is also a greedy $\Delta$-approximation algorithm for covering problems with submodular cost \cite{Koufogiannakis13}. 
%}

%\subsubsection{Applications}
There are several  applications for submodular \bmatching \  and \bedgecover \ :  content spread maximization \cite{Chaoji12}, peptide identification in tandem mass spectrometry \cite{Bai16,Bai19}, word alignment \cite{Lin11},  and diversity maximizing assignment \cite{Ahmadi19,Dickerson18}.


